Don't Blame the Large Language Model: How Agent Harness Evolution Shapes Coding Agent Quality

Coding agents, autonomous systems that use large language models (LLMs) to resolve software engineering tasks, rely on agent harness: a middleware layer in between a developer and a large language model that orchestrates system prompts, tool execution, context management, and iterative reasoning loops. While these agent harnesses evolve at extreme velocities, no study has examined how this evolution affects agent quality (i.e., effectiveness and efficiency) over time. Practitioners regularly report quality regressions after agent harness updates, yet consistently attribute them to the underlying model rather than the harness itself. In this paper, we address this gap by conducting the first controlled longitudinal study that isolates the agent harness contribution. Unlike prior work that fixes the agent harness and varies the model, we fix the model and vary only the agent harness, evaluating 35 sequential releases to measure their impact on agent effectiveness and efficiency. We first empirically study the development and release evolution of five major open-source agent harnesses (i.e., Codex, Qwen Code, Gemini, OpenCode, and OpenHands), revealing extreme release velocities exceeding two releases per day and thousands of issues within months. We then perform a controlled deep dive into 35 sequential releases of the Qwen Code CLI, evaluating each against 50 stratified SWE-bench Verified tasks while holding the underlying LLM constant. We trace the resulting quality fluctuations to specific development patterns and architectural components, and illustrate our findings with concrete qualitative evidence linking individual pull requests to measured quality shifts.

==> sections/rq2_tables.tex <==
\begin{table*}[t]
\centering
\caption{Absolute (Raw) statistical results. Significant values ($p<0.05$) are highlighted.}
\label{tab:rq2-raw-stats}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll cccccc}
\toprule
Factor & Category & Res. $d$ & Res. $p$ & Tok. $d$ & Tok. $p$ & Tool $d$ & Tool $p$ \\
\midrule
`days\_since\_prev` & Release Cadence & 0.467 & 0.1471 & 0.030 & 0.9264 & 0.000 & 1.0000 \\
`total\_commits` & Dev. Activity & 0.167 & 0.6250 & -0.601 & \textbf{0.0138} & -0.400 & 0.3893 \\
`pr\_count` & Dev. Activity & 0.350 & 0.2767 & -0.217 & 0.3840 & -0.550 & 0.2187 \\
`unique\_authors` & Dev. Activity & 0.050 & 0.9120 & -0.482 & \textbf{0.0476} & -0.450 & 0.3252 \\
`total\_churn` & Code Churn & 0.300 & 0.3676 & -0.105 & 0.6851 & -0.200 & 0.7302 \\
`total\_additions` & Code Churn & 0.400 & 0.2198 & -0.231 & 0.3539 & -0.300 & 0.5556 \\
`total\_deletions` & Code Churn & 0.267 & 0.4278 & 0.140 & 0.5820 & -0.150 & 0.8057 \\
`mean\_pr\_size` & Code Churn & 0.267 & 0.4278 & 0.091 & 0.7281 & 0.100 & 0.9048 \\
`max\_pr\_size` & Code Churn & 0.300 & 0.3676 & 0.007 & 1.0000 & -0.100 & 0.9048 \\
`total\_changed\_files` & Code Churn & 0.417 & 0.1927 & -0.126 & 0.6223 & -0.600 & 0.1905 \\
`feat\_churn\_ratio` & Change Composition & 0.533 & 0.0793 & -0.573 & \textbf{0.0149} & -0.900 & \textbf{0.0365} \\
`fix\_churn\_ratio` & Change Composition & 0.333 & 0.2992 & -0.496 & \textbf{0.0421} & -0.500 & 0.2857 \\
`refactor\_churn\_ratio` & Change Composition & -0.400 & 0.1013 & 0.238 & 0.2089 & 0.100 & 0.8668 \\
`fix\_pr\_ratio` & Change Composition & 0.333 & 0.2989 & -0.399 & 0.1034 & -0.450 & 0.3252 \\
`feat\_pr\_ratio` & Change Composition & 0.450 & 0.1404 & -0.489 & \textbf{0.0379} & -0.600 & 0.1761 \\
`fix\_to\_feat\_ratio` & Change Composition & 0.217 & 0.5076 & -0.112 & 0.6600 & -0.150 & 0.8041 \\
`mean\_time\_to\_merge\_hours` & Process Quality & 0.433 & 0.1806 & -0.035 & 0.9078 & -0.100 & 0.9048 \\
`needs\_triage\_count` & Project Health & 0.250 & 0.4150 & -0.832 & \textbf{0.0005} & -0.750 & 0.0733 \\
`issues\_opened` & Project Health & 0.417 & 0.1924 & 0.098 & 0.7058 & -0.250 & 0.6228 \\
`bug\_count` & Project Health & 0.800 & \textbf{0.0096} & -0.545 & \textbf{0.0243} & -0.600 & 0.1706 \\
`feature\_count` & Project Health & 0.617 & \textbf{0.0311} & -0.455 & 0.0509 & -0.400 & 0.3812 \\
`bug\_to\_feature\_ratio` & Project Health & 0.750 & \textbf{0.0061} & -0.664 & \textbf{0.0036} & -0.650 & 0.1248 \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[t]
\centering
\caption{Delta ($\Delta$) statistical results tracking immediate release transitions . Significant values ($p<0.05$) are highlighted.}
\label{tab:rq2-delta-stats}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll cccc cccc cccc}
\toprule
 & & \multicolumn{4}{c}{Resolve Rate} & \multicolumn{4}{c}{Token Consumption} & \multicolumn{4}{c}{Tool Calls} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
Factor & Category & $\rho$ & $p$ & MW $p$ & $d$ & $\rho$ & $p$ & MW $p$ & $d$ & $\rho$ & $p$ & MW $p$ & $d$ \\
\midrule
`mean\_time\_to\_merge\_hours` & process & 0.296 & 0.089 & 0.456 & 0.265 & -0.246 & 0.161 & 0.755 & 0.125 & -0.276 & 0.114 & 0.232 & 0.393 \\
`mean\_pr\_size` & churn & 0.258 & 0.141 & 0.805 & 0.102 & -0.441 & \textbf{0.009} & 0.081 & 0.583 & -0.484 & \textbf{0.004} & 0.054 & 0.607 \\
`unique\_authors` & activity & -0.249 & 0.155 & 0.054 & -0.633 & -0.021 & 0.907 & 0.698 & -0.146 & -0.082 & 0.644 & 0.600 & 0.179 \\
`fix\_churn\_ratio` & composition & -0.243 & 0.165 & 0.383 & -0.306 & 0.339 & 0.050 & \textbf{0.008} & -0.833 & 0.255 & 0.145 & 0.336 & -0.321 \\
`feat\_pr\_ratio` & composition & 0.174 & 0.325 & 0.902 & 0.061 & -0.012 & 0.947 & 0.755 & 0.125 & -0.076 & 0.668 & 0.954 & -0.036 \\
`pr\_count` & activity & -0.171 & 0.332 & 0.096 & -0.551 & -0.126 & 0.479 & 1.000 & -0.021 & -0.115 & 0.517 & 0.353 & 0.304 \\
`feat\_churn\_ratio` & composition & 0.160 & 0.367 & 0.710 & 0.143 & 0.088 & 0.620 & 0.662 & 0.167 & 0.138 & 0.436 & 0.281 & -0.357 \\
`total\_commits` & activity & -0.156 & 0.379 & 0.159 & -0.469 & -0.098 & 0.583 & 0.897 & -0.062 & -0.106 & 0.549 & 0.463 & 0.250 \\
`bug\_to\_feature\_ratio` & health & 0.145 & 0.414 & 0.535 & 0.225 & -0.018 & 0.918 & 0.244 & 0.396 & -0.033 & 0.854 & 0.861 & 0.071 \\
`refactor\_churn\_ratio` & composition & -0.129 & 0.467 & 0.104 & -0.490 & -0.276 & 0.114 & 0.259 & 0.333 & -0.070 & 0.695 & 0.267 & 0.321 \\
`total\_deletions` & churn & -0.129 & 0.469 & 0.165 & -0.469 & -0.351 & \textbf{0.042} & 0.282 & 0.375 & -0.329 & 0.058 & 0.152 & 0.464 \\
`fix\_to\_feat\_ratio` & composition & 0.117 & 0.509 & 0.406 & 0.286 & -0.058 & 0.745 & 0.746 & -0.125 & -0.108 & 0.541 & 0.602 & 0.179 \\
`feature\_count` & health & -0.116 & 0.516 & 0.405 & -0.286 & -0.078 & 0.661 & 0.650 & -0.167 & -0.108 & 0.544 & 0.520 & 0.214 \\
`bug\_count` & health & 0.068 & 0.701 & 0.749 & -0.122 & 0.005 & 0.977 & 0.698 & -0.146 & -0.039 & 0.825 & 0.562 & 0.196 \\
`max\_pr\_size` & churn & 0.043 & 0.810 & 0.535 & -0.225 & -0.290 & 0.096 & 0.414 & 0.292 & -0.351 & \textbf{0.042} & 0.121 & 0.500 \\
`days\_since\_prev` & cadence & 0.043 & 0.811 & 0.628 & -0.191 & -0.098 & 0.586 & 0.524 & -0.250 & -0.122 & 0.498 & 0.209 & 0.429 \\
`total\_churn` & churn & 0.036 & 0.841 & 0.456 & -0.265 & -0.291 & 0.095 & 0.491 & 0.250 & -0.312 & 0.072 & 0.232 & 0.393 \\
`needs\_triage\_count` & health & -0.031 & 0.861 & 0.367 & -0.306 & -0.025 & 0.887 & 0.603 & -0.188 & -0.044 & 0.804 & 0.637 & 0.161 \\
`total\_changed\_files` & churn & -0.024 & 0.894 & 0.383 & -0.306 & -0.267 & 0.127 & 0.491 & 0.250 & -0.258 & 0.141 & 0.336 & 0.321 \\
`fix\_pr\_ratio` & composition & 0.018 & 0.920 & 0.902 & 0.061 & 0.084 & 0.636 & 0.282 & -0.375 & 0.007 & 0.968 & 1.000 & 0.000 \\
`issues\_opened` & health & -0.006 & 0.971 & 0.441 & -0.265 & -0.014 & 0.939 & 0.332 & -0.333 & -0.074 & 0.679 & 0.602 & 0.179 \\
`total\_additions` & churn & -0.003 & 0.987 & 0.318 & -0.347 & -0.233 & 0.184 & 0.573 & 0.208 & -0.281 & 0.108 & 0.189 & 0.429 \\
\bottomrule
\end{tabular}}
\end{table*}


==> sections/rq3_table_base.tex <==
\begin{table}[htbp]
\centering
\caption{Significant Architectural Component signals surviving strict empirical filtering (Base Metrics).}
\label{tab:rq3-base}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{c l l l l r r r}
\toprule
\# & Perspective & Dimension & Component & Metric & Spearman $\rho$ & $p$ & Partial S. $\rho$ \\
\midrule
A1 & Absolute & Effectiveness & Extensibility & additions & +0.288 & 0.094 & +0.240 \\
A2 & Absolute & Token Consumption & Context Mgmt & binary & -0.320 & 0.061 & -0.361 \\
A3 & Absolute & Token Consumption & Extensibility & additions & +0.317 & 0.063 & +0.306 \\
D1 & Delta & Effectiveness & LLM Provider & volume & -0.435 & 0.009 & -0.324 \\
D2 & Delta & Effectiveness & UI & volume & -0.355 & 0.036 & -0.161 \\
D3 & Delta & Effectiveness & Persistence & binary & -0.339 & 0.046 & -0.076 \\
D4 & Delta & Token Consumption & Persistence & volume & +0.308 & 0.072 & +0.289 \\
D5 & Delta & Token Consumption & UI & deletions & +0.293 & 0.088 & +0.276 \\
D6 & Delta & Tool Calls & Context Mgmt & binary & -0.320 & 0.061 & -0.253 \\
\bottomrule
\end{tabular}
% }
\end{table}


==> sections/rq3_tables.tex <==
\begin{table*}[t]
\centering
\caption{Significant Architectural Component signals surviving strict empirical filtering (Base Metrics).}
\label{tab:rq3-base}
\resizebox{\textwidth}{!}{
\begin{tabular}{c l l l l r r r l}
\toprule
\# & Perspective & Dimension & Component & Metric & $\rho$ & $p$ & Partial $\rho$ & Verdict \\
\midrule
A1 & Absolute & Effectiveness & Extensibility & additions & +0.288 & 0.094 & +0.240 & Genuine \\
A2 & Absolute & Token Eff. & Context Mgmt & binary & -0.320 & 0.061 & -0.361 & Genuine (strengthens) \\
A3 & Absolute & Token Eff. & Extensibility & additions & +0.317 & 0.063 & +0.306 & Genuine \\
D1 & Delta & Effectiveness & LLM Provider & volume & -0.435 & 0.009 & -0.324 & Genuine — headline result \\
D2 & Delta & Effectiveness & UI & volume & -0.355 & 0.036 & -0.161 & Confound (55% drop) \\
D3 & Delta & Effectiveness & Persistence & binary & -0.339 & 0.046 & -0.076 & False positive \\
D4 & Delta & Token Eff. & Persistence & volume & +0.308 & 0.072 & +0.289 & Genuine \\
D5 & Delta & Token Eff. & UI & deletions & +0.293 & 0.088 & +0.276 & Genuine \\
D6 & Delta & Interaction Eff. & Context Mgmt & binary & -0.320 & 0.061 & -0.253 & Genuine \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[t]
\centering
\caption{Extended Absolute Analysis: File-operation and Commit-type signals tracking continuous project growth.}
\label{tab:rq3-ext-abs}
\resizebox{\textwidth}{!}{
\begin{tabular}{c l l l r r r l}
\toprule
\# & Dimension & Component & Metric & $\rho$ & $p$ & Partial $\rho$ & Verdict \\
\midrule
AE1 & Effectiveness & Config & feat\_churn & +0.318 & 0.062 & +0.290 & Genuine \\
AE2 & Effectiveness & Security & fix\_ratio & +0.318 & 0.063 & +0.289 & Genuine \\
AE3 & Effectiveness & Context Mgmt & feat\_ratio & +0.316 & 0.064 & +0.294 & Genuine \\
AE4 & Effectiveness & Extensibility & feat\_churn & +0.284 & 0.098 & +0.254 & Genuine \\
AE5 & Token Eff. & LLM Provider & add\_del\_ratio & +0.490 & 0.003 & +0.492 & Strongest finding \\
AE6 & Token Eff. & Extensibility & fix\_churn & +0.375 & 0.027 & +0.356 & Genuine \\
AE7 & Token Eff. & UI & add\_del\_ratio & +0.369 & 0.029 & +0.369 & Genuine (zero confound) \\
AE8 & Token Eff. & Context Mgmt & add\_del\_ratio & -0.346 & 0.042 & -0.392 & Genuine (strengthens) \\
AE9 & Interaction Eff. & LLM Provider & fix\_ratio & +0.367 & 0.030 & +0.373 & Genuine \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[t]
\centering
\caption{Extended Delta Analysis: Immediate component transitions negating maturity confound.}
\label{tab:rq3-ext-delta}
\resizebox{\textwidth}{!}{
\begin{tabular}{c l l l r r r l}
\toprule
\# & Dimension & Component & Metric & $\rho$ & $p$ & Partial $\rho$ & Verdict \\
\midrule
DE1 & Effectiveness & UI & refactor\_churn & -0.391 & 0.020 & -0.276 & Genuine \\
DE2 & Effectiveness & LLM Provider & add\_del\_ratio & -0.336 & 0.049 & -0.221 & Genuine \\
DE3 & Effectiveness & Extensibility & files\_added\_ratio & -0.285 & 0.097 & -0.161 & Weak/confound \\
DE4 & Token Eff. & Persistence & add\_del\_ratio & +0.353 & 0.037 & +0.332 & Genuine \\
DE5 & Token Eff. & Security & fix\_ratio & +0.346 & 0.042 & +0.327 & Genuine \\
DE6 & Interaction Eff. & Persistence & refactor\_churn & +0.345 & 0.042 & +0.334 & Genuine \\
DE7 & Interaction Eff. & Security & fix\_ratio & +0.341 & 0.045 & +0.339 & Genuine \\
DE8 & Interaction Eff. & Config & refactor\_churn & +0.331 & 0.052 & +0.320 & Genuine \\
DE9 & Interaction Eff. & UI & refactor\_churn & +0.298 & 0.083 & +0.291 & Genuine \\
\bottomrule
\end{tabular}}
\end{table*}


==> sections_old/discussion_bak.tex <==
%% ============================================================================
%% SECTION 8: DISCUSSION
%% ============================================================================
\section{Discussion}
\label{sec:discussion}

We synthesize the findings from RQ0--RQ3, offer a likely explanation for the Scaffolding Paradox grounded in the absence of agentic regression testing, and distill implications for practitioners, researchers, and the emerging field of agentic software engineering. \hao{why so wordy in this section?} \hao{rewrite this section following the same writing style as the results section: first sentence conveys the key message before elaborating details; connect with our findings instead of general knowledge; elaborate more details/dig deeper. You can also check other papers from the lab. Currently, the key messages are buried with a strong AI smell}

\subsection{The Scaffolding Paradox: More Code Does Not Mean Better Agents}
\label{sec:disc:paradox}

Our longitudinal analysis challenges the prevailing assumption that continuously iterating on an agent's scaffolding leads to improved benchmark performance. By isolating the foundation model, we demonstrated that scaffolding evolution, characterized by increasing prompt lengths, additional feature abstractions, and growing context overhead (RQ1), often yields diminishing or negative returns. This pattern mirrors classical observations in software engineering: Lehman's law of increasing complexity~\cite{lehman1980programs} predicts that actively developed software grows more complex over time, and Parnas~\cite{parnas1994software} argued that such accumulated complexity degrades software quality unless actively counteracted. Brooks~\cite{brooks1995mythical} similarly observed that adding complexity to a late software project tends to make it later.

In the agentic context, this technical debt manifests as wasted API tokens, inflated tool call counts, and stagnant resolve rates. The scaffolding's growing prompt payload and extended conversation turns impose a compounding cost on every inference call, while the additional complexity fails to improve, and sometimes harms, the LLM's ability to reason about the task. Building effective autonomous agents is therefore not solely a prompt engineering challenge but a continuous software architecture problem in which component complexity must be balanced against the finite capacity of the LLM's context window and reasoning ability.

Our findings provide empirical evidence that Lehman's laws~\cite{lehman1980programs}, originally formulated for traditional software systems, apply with particular force to agentic scaffolding. Token consumption and tool calls increase monotonically across releases (RQ1), reflecting growing internal complexity (\emph{Increasing Complexity}). The flat resolve rate despite increasing investment is consistent with Lehman's prediction that quality declines unless actively maintained (\emph{Declining Quality}). The high proportion of one-time contributors (48--68\%, RQ0) suggests that the system changes faster than contributors can maintain familiarity with it (\emph{Conservation of Familiarity}).

The Scaffolding Paradox also has economic implications. With cloud API pricing tied directly to token consumption, and subscription-based plans subject to additional rate constraints such as hourly and weekly usage limits, the near-doubling of token usage observed between early and late releases (RQ1) translates to a proportional increase in operational cost per task, without any corresponding improvement in task resolution. For organizations deploying coding agents at scale, scaffolding bloat represents a significant and often invisible cost driver.

\subsection{The Absence of Agentic Regression Testing}
\label{sec:disc:agentic-qa}

Our findings across RQ1--RQ3 raise a more fundamental question: \emph{why} do these regressions persist? The concrete examples documented throughout this paper (the search tool rewrites that doubled token consumption in v0.1.4$\to$v0.1.5, the streaming overhauls that tripled it in v0.2.3$\to$v0.3.0, and the converter changes that degraded resolve rates in v0.4.1$\to$v0.5.0) all share a common characteristic: every one of these changes passed the project's full CI/CD pipeline. The regressions were not introduced by careless development; they were introduced by a development process that appears structurally incapable of detecting them.

The development activities that drive the Scaffolding Paradox (feature additions, bug fixes, refactoring) are themselves sound engineering practices. Their behavioral and functional correctness is well-covered by conventional testing: unit tests verify that individual tools produce correct outputs, integration tests confirm that the CLI executes without crashing in sandboxed environments, and end-to-end tests validate that tool calls complete successfully against real files. These tests are necessary and valuable, but they are fundamentally insufficient for a critical class of regressions: \emph{performance regressions that manifest not in whether the code works, but in how well the agent performs its task.}

A search tool rewrite may pass every unit test (each function returns the correct result) while simultaneously changing the volume and format of tool output in ways that degrade the LLM's reasoning. A context management expansion may pass every integration test (the CLI does not crash) while inflating the prompt payload enough to double token consumption. These are not bugs in the traditional sense; they are emergent behavioral regressions that arise from the interaction between the scaffolding and the LLM, and they are \emph{not catchable} by unit tests, integration tests, or end-to-end functional tests. Detecting them requires evaluating the agent's actual task performance (resolve rate, token consumption, tool call efficiency) on representative benchmarks.

To assess whether such evaluation exists, we conducted a systematic inspection of the \qwen CLI's CI/CD pipelines, test suites, and GitHub Actions workflows by manually examining all YAML workflow files in the \texttt{.github/workflows/} directory and all test files in \texttt{src/\_\_tests\_\_/} and \texttt{integration-tests/}.\footnote{Inspection conducted on the \texttt{main} branch of \url{https://github.com/QwenLM/qwen-code} as of March~2026.}

The project maintains an extensive test suite of over 300 unit test files (using Vitest) and a dedicated \texttt{integration-tests/} directory. The unit tests validate tool correctness (e.g., ``does the edit tool modify the file?''), configuration parsing, UI component rendering, authentication flows, and MCP protocol compliance. Integration tests spin up the CLI in sandboxed environments (Docker, Podman, or unsandboxed) and verify that tool calls execute successfully against real files. The CI pipeline (\texttt{ci.yml}) runs on every pull request and push to \texttt{main}, executing lint checks, unit tests across three Node.js versions and three operating systems, code coverage reporting, and CodeQL security analysis. E2E tests (\texttt{e2e.yml}) run on pushes to \texttt{main} and merge queue entries.

Despite this comprehensive functional test infrastructure, the \textbf{public} repository contains \textbf{no automated regression testing for agentic performance} (we cannot rule out the existence of internal evaluation pipelines not reflected in the public repository). No CI workflow evaluates the agent against SWE-bench, HumanEval, or any other coding benchmark, so a pull request that reduces resolve rate from 42\% to 20\% would pass all automated checks. No test asserts that mean tokens per task remains below a budget, making a change that doubles token consumption invisible to the CI pipeline. No test monitors the number or distribution of tool calls per task, so a change that traps the agent in fruitless edit-test-read loops goes undetected. And no test examines the agent's intermediate reasoning steps for pathological patterns such as repetitive loops or premature termination.

The project shows some awareness of this gap. An \texttt{eval.yml} workflow exists but is a stub that sets up Node.js and Python without running any evaluation. A \texttt{terminal-bench.yml} workflow runs only two tasks (a trivial ``hello world'' file creation and a single SWE-bench instance), is triggered only on \texttt{feat/tbench*} branches and releases, \emph{not} on pull requests or pushes to \texttt{main}, and measures only pass/fail without recording token consumption, tool call counts, or efficiency metrics. The agent statistics module (\texttt{agent-statistics.ts}) correctly \emph{counts} tokens and tool calls, but no CI job \emph{checks} whether those counts have regressed. The infrastructure for measurement exists; the infrastructure for \emph{enforcement} does not.

This absence of agentic regression testing \bram{doesn't sound very sure?} \oussama{I think this comment was there because of ``likely'' that was removed} \hao{remove `likely' won't solve the problem, what is the evidence (I mean direct evidence)? Also, we never explain what agentic regression testing is and how to do so?} \hao{how many claims here have evidence support? any claims are based on our findings instead of general knowledge?} \oussama{In this paragraph, we are already including some real cases from our qualitative analysis and referring to findings.} \hao{could you tighten the writing and make it clear for ALL paragraphs?} is a key factor behind the patterns documented throughout this paper at both the project and architecture levels. Token consumption and tool calls increase monotonically (RQ1); the absence of token budget assertions in the CI pipeline means that no automated check existed to prevent their inflation before release. the 139\% token spike in v0.1.5 and the 182\% spike in v0.3.0 both passed all CI checks. Fix-heavy releases inflate costs (Finding~17, RQ2), likely because developers add error-handling and fallback logic without visibility into its impact on token budgets, and feature additions improve resolve rate but increase costs (Finding~12) because the trade-off is not systematically and automatically quantified before merge. High-risk components like the LLM Provider and Context Management cause regressions when modified (Findings~20, 23, RQ3), likely because their effects on agent behavior cannot be detected with functional tests alone; these components affect \emph{how} the model reasons, not whether the code compiles.

We cannot establish a definitive causal link \hao{this just conflicts with the first sentence of the previous paragraph} between the absence of agentic regression testing and the Scaffolding Paradox. Other factors, such as the inherent difficulty of predicting LLM behavior or the stochastic nature of agent execution, may also contribute. However, the evidence is strongly suggestive as every concrete example of performance degradation we documented passed the project's full functional test suite, and the specific kinds of regressions we observe \bram{bug resolution = ability to perform a task = feature, so should be a functional test?} \oussama{not sure what this means, I already mentioned that it passes the functional test suite. And yes a functional test represents the ability of performing a task, that is bug resolution in our case.} are precisely the kinds that the project's existing tests do not cover (e.g., token inflation, tool call inflation); resolve rate regressions could in principle be caught by functional tests, but only if those tests evaluate task completion at scale on representative benchmarks, which the project's CI does not. At minimum, the absence of performance regression testing means that these regressions \emph{could not have been} detected before release, regardless of whether they would have been prevented. A regression testing pipeline that ensures each release performs at least as well as the previous version, in terms of resolve rate, token efficiency, and tool call overhead, would provide the missing feedback loop that the current development process lacks.

\subsection{Agentic CLIs as a New Category of Software}
\label{sec:disc:new-category}

Our findings suggest that agentic CLIs and agent-based IDEs represent a fundamentally \emph{new category of software} that challenges existing quality assurance paradigms. Unlike traditional CLI tools or IDE plugins, where functional correctness (e.g., ``does the command produce the right output?'') is the primary quality dimension, agentic scaffolding must satisfy a \emph{multi-faceted quality} model in which functional correctness is necessary but far from sufficient.

In traditional software, if the code compiles, passes its tests, and produces correct outputs, it is generally considered ready for release. Agentic scaffolding breaks this assumption. A release can be functionally correct in every conventional sense (every tool returns the right result, every API call succeeds, every UI component renders properly) while simultaneously degrading the agent's task performance, inflating its resource consumption, or trapping it in unproductive reasoning loops. Quality in this new category of software is inherently multi-dimensional: it spans functional correctness, task effectiveness (resolve rate), resource efficiency (token consumption, tool calls), reasoning quality (trajectory patterns), and economic cost.

This multi-faceted quality challenge has a noteworthy parallel in blockchain and smart contract systems~\cite{chen2020survey, atzei2017survey}. In blockchain software, functional correctness (``does the contract execute?'') is likewise insufficient; developers must additionally track and optimize gas consumption, the computational cost of executing transactions on-chain, because gas directly determines economic viability. A smart contract that is functionally correct but gas-inefficient may be unusable in practice, just as an agentic scaffolding that is functionally correct but token-inefficient imposes unsustainable operational costs. In both domains, there is no single ``functional requirement'' that captures quality; instead, developers must continuously monitor and optimize across multiple performance dimensions that are invisible to conventional testing. The token economy of agentic systems and the gas economy of blockchain systems share a core property: \emph{resource consumption is a first-class quality attribute}, not merely an implementation detail.

These systems are fundamentally different from traditional tools because the user of the scaffolding is an LLM whose behavior is sensitive to subtle changes in prompt structure, tool output format, and context composition. No amount of unit testing can anticipate these sensitivities. Studying, characterizing, and developing appropriate QA methodologies for this new category of software is an important direction for the software engineering research community.

\subsection{Toward Agentic Quality Assurance}
\label{sec:disc:toward-agentic-qa}

Our findings argue for a new category of software quality assurance that we term \emph{Agentic QA}: regression testing that evaluates the agent's actual behavior (e.g., task performance, resource efficiency, reasoning quality) rather than merely verifying that the underlying code executes correctly.

The core principle of Agentic QA is that \emph{every release should perform at least as well as the previous version}. Features, bug fixes, and refactoring are all valuable development activities, and their functional correctness is appropriately validated by unit and integration tests. But their impact on agent performance (e.g., whether a bug fix inadvertently inflates token consumption, whether a feature addition degrades resolve rate, whether a refactoring disrupts established reasoning pathways) must be validated separately through performance regression testing on representative benchmarks.

An Agentic QA pipeline would include benchmark regression gates that run a representative subset of tasks from an established benchmark (e.g., 50 stratified SWE-bench Verified tasks, as in our study) on every PR or nightly build, flagging any release where resolve rate drops beyond a configurable threshold relative to the previous version. It would also include token budget assertions that check whether mean token consumption per task exceeds a specified budget; our data shows that the most efficient release (v0.1.4, 121K tokens) achieved the highest resolve rate, suggesting that tighter token budgets may actually \emph{improve} agent quality by preventing wasteful reasoning loops. Tool call efficiency monitoring would track the mean and distribution of tool calls per task, flagging releases where tool call counts increase significantly, as elevated tool calls correlate with the agent being trapped in unproductive exploration patterns (Finding~8). Finally, reasoning trajectory analysis would examine the agent's intermediate steps for pathological patterns such as repetitive edit-test-read loops, premature termination, or context window saturation, which are invisible to token-level metrics but directly explain why more tokens do not yield better results.

Such a pipeline need not be expensive. Our evaluation of 50 tasks across two runs per version required approximately 10 hours of GPU time per release on a dual-GPU server. A smaller diagnostic subset of 10--20 tasks could provide meaningful regression signal in under 3 hours, making it feasible as a nightly or per-milestone gate.

% \subsection{Actionable Guidelines for Scaffolding Developers}
% \label{sec:disc:practitioners}

%% \subsection{Actionable Guidelines for Scaffolding Developers}
%% \label{sec:disc:practitioners}
%%
%% In the absence of Agentic QA pipelines, scaffolding developers should adopt the following guidelines derived from the component-level analysis in RQ3:
%%
%% \begin{itemize}[leftmargin=*]
%%     \item \textbf{Guideline 1: Modify the LLM Provider Layer Incrementally.} Our data shows that large modifications to the LLM Provider carry immediate regression risk (Finding~15), even though additive changes are beneficial long-term (Finding~11). Scaffolding developers should separate prompt formatting, model adapters, and streaming handlers into modular interfaces, and modify them independently to minimize disruption.
%%     \item \textbf{Guideline 2: Treat Context Management as a Budget, Not a Feature.} Expanding the Context Management layer correlates with decreased token efficiency (Finding~12). Every additional piece of information added to the LLM's context window (tool schemas, conversation history, memory summaries) competes for the model's attention. Developers should apply strict budgeting to context, removing low-value information before adding new content.
%%     \item \textbf{Guideline 3: Prioritize Targeted Security Fixes.} Unlike broad feature additions or refactoring, surgical bug fixes within the Security domain are the only modification pattern that consistently improves operational efficiency without introducing regressions (Finding~13). This suggests that security-related improvements, which typically enforce tighter execution boundaries, help the agent avoid wasteful exploration.
%%     \item \textbf{Guideline 4: Consolidate Changes and Remove Dead Code.} PR consolidation reduces token costs (Finding~7), and code deletions directly lower token consumption (Finding~8). Conversely, fragmented micro-commits and fix-heavy transitions inflate costs (Finding~9). Scaffolding teams should favor fewer, larger, well-tested PRs and actively prune deprecated code paths.
%% \end{itemize}
%%
%% \subsection{Implications for Release Engineering}
%% \label{sec:disc:release}
%%
%% The hyper-churn release patterns documented in RQ0, with some frameworks averaging over two releases per day, represent a qualitatively different release engineering regime from what has been studied in prior work on rapid release cycles~\cite{adams2016release}. The lack of correlation between release cadence and performance (Finding~6) indicates that the problem is not release frequency per se, but rather the nature of the changes shipped and the absence of performance gates. Slowing down releases alone will not improve agent quality; what is needed is instrumentation that makes the agentic cost of each change visible before it ships.
%%
%% The near-instantaneous PR review times (under 4 hours for three of five frameworks, RQ0) combined with the negative effects of fragmented changes (Finding~7) suggest that the current development workflow prioritizes speed over coherence. Adopting release trains, where changes are batched into periodic, well-tested releases, could mitigate the fragmentation overhead we observe, particularly if combined with Agentic QA gates at each release boundary.
%%
%% \subsection{Implications for Researchers and Benchmarking}
%% \label{sec:disc:researchers}
%%
%% For the academic community, our findings necessitate a methodological shift in how coding agents are evaluated:
%%
%% \paragraph{Version Control in Benchmarking.} Future studies that benchmark coding agents on \swebench or similar benchmarks must report the specific scaffolding version used, not merely the underlying LLM. Our data shows that the same model can exhibit resolve rates ranging from 20\% to 42\% depending solely on the scaffolding version (RQ1). A benchmark result that does not specify the scaffolding version is not reproducible and may not be comparable to other results.
%%
%% \paragraph{Longitudinal Evaluation.} Single-snapshot evaluations, which are the current norm, mask the substantial version-to-version variation we document. We advocate for longitudinal evaluation protocols that track performance across multiple releases to distinguish stable improvements from transient fluctuations.
%%
%% \paragraph{Efficiency as a First-Class Metric.} Current benchmarking practices focus almost exclusively on resolve rate. Our findings demonstrate that efficiency metrics (token consumption, tool calls) reveal important dynamics that resolve rate alone misses: later versions consume nearly double the tokens without improving effectiveness (RQ1). Reporting efficiency alongside effectiveness provides a more complete picture of agent quality.
%%
%% \paragraph{Scaffolding as an Independent Variable.} Our controlled experimental design, holding the LLM constant while varying the scaffolding, demonstrates that the scaffolding is a significant independent variable in agent performance. Future work should explore this variable systematically, including cross-scaffolding comparisons where the same model is evaluated under different agent frameworks.
%%
%% \paragraph{A New Category of Software to Study.} Agentic CLIs and agent-based IDEs constitute a new and rapidly growing category of software that differs fundamentally from traditional development tools. Their multi-faceted quality model, spanning functional correctness, task effectiveness, resource efficiency, and reasoning quality, demands new empirical methodologies, new quality metrics, and new testing frameworks. The software engineering research community should prioritize the study of these systems and their evolution patterns, and the development of appropriate QA practices for them.

